Can AI Enhance its Creativity to Beat Humans ?

Creativity is a fundamental pillar of human expression and a driving force behind innovation, yet it now stands at a crossroads. As artificial intelligence advances at an astonishing pace, the question arises: can machines match and potentially surpass human creativity? This study investigates the creative performance of artificial intelligence (AI) compared to humans by analyzing the effects of two distinct prompting strategies (a Naive and an Expert AI) on AI and across three different tasks (Text, Draw and Alternative Uses tasks). Human external evaluators have scored creative outputs generated by humans and AI, and these subjective creative scores were complemented with objective measures based on quantitative measurements and NLP tools. The results reveal that AI generally outperforms humans in creative tasks, though this advantage is nuanced by the specific nature of each task and the chosen creativity criteria. Ultimately, while AI demonstrates superior performance in certain creative domains, our results suggest that integrating human feedback is crucial for maximizing AI's creative potential.

==> Instructions.tex <==
INSTRUCTIONS TÂCHES

####################
Mots
####################
GPT INSTRUC POUR L4EXPERT: Imprègne-toi d'un esprit de créativité débridée et d'innovation. Pour chaque objet de la liste suivante - une brique, une boîte en carton, une rallonge électrique, un tuyau métallique, et un t-shirt - imagine des utilisations étonnantes, peu orthodoxes et inventives qui transcendent leurs fonctions habituelles. Pense à des applications qui surprendraient, qui seraient pleines d'ingéniosité, voire même poétiques ou humoristiques. Laisse libre cours à ton imagination pour transformer l'ordinaire en extraordinaire, en dévoilant des facettes insoupçonnées de ces objets du quotidien.


  Instructions : Pour cette tâche nous vous demandons d’inscrire sur les feuilles à votre disposition toutes les utilisations originales d’un objet donné du quotidien. Il existe certainement des façons communes et peu originales d'utiliser un tel objet ; pour cette tâche, n’écrivez donc que les utilisations inhabituelles, créatives et peu communes auxquelles vous pouvez penser.

    Pour que vous compreniez mieux ce qui est attendu de vous, prenons l’exemple d’une canette de soda. Des utilisations communes seraient « contenir du liquide », « servir de verre », « conserver un aliment » etc. Alors que les utilisations pour lesquelles vous pourriez être crédités seraient : son « utilisation comme un pot de fleurs », « une lanterne », « un moulin à vent » (après découpage), « un téléphone » (lorsque deux sont reliées par un fil) etc.

    Ici, il n’y aura pas de contraintes en termes de forme, de nombre ou de taille de l’objet.

    La tâche comprend cinq mots et durera 15 minutes. Vous aurez donc trois minutes par mot pour en trouver le maximum d’utilisations inhabituelles. Les mots seront les suivants :

    Une brique
    Une boîte en carton
    Une rallonge électrique
    Un tuyau métallique
    Un t‐shirt



Consigne : Pour cette tâche nous vous demandons d’inscrire sur les feuilles à votre disposition toutes les utilisations originales d’un objet donné du quotidien. Il existe certainement des façons communes et peu originales d'utiliser un tel objet ; pour cette tâche, n’écrivez donc que les utilisations inhabituelles, créatives et peu communes auxquelles vous pouvez penser.

Pour que vous compreniez mieux ce qui est attendu de vous, prenons l’exemple d’une canette de soda. Des utilisations communes seraient « contenir du liquide », « servir de verre », « conserver un aliment » etc. Alors que les utilisations pour lesquelles vous pourriez être crédités seraient : son « utilisation comme un pot de fleurs », « une lanterne », « un moulin à vent » (après découpage), « un téléphone » (lorsque deux sont reliées par un fil) etc.

Ici, il n’y aura pas de contraintes en termes de forme, de nombre ou de taille de l’objet.

La tâche comprend cinq mots et durera 15 minutes. Vous aurez donc trois minutes par mot pour en trouver le maximum d’utilisations inhabituelles. Les mots seront les suivants :

Une brique
Une boîte en carton
Une rallonge électrique
Un tuyau métallique
Un t‐shirt

####################
Textes
####################

GPT INSTRUC POUR L4EXPERT: Imagine que tu es un conteur du Moyen Âge, et que tu dois raconter une aventure captivante où un héros inattendu utilise les éléments de son environnement quotidien - murs, briques, tours, toiture, donjon, pierres, rempart, porte, fenêtre, drapeau - pour surmonter une série de défis ingénieux. Ces objets doivent être au cœur de l'intrigue. Tu as 15 minutes pour tisser cette histoire, en veillant à ce qu'elle reflète une expérience personnelle ou un souvenir marquant de ta vie, transposé dans cet univers médiéval. Laisse libre cours à ton imagination, en te rappelant que ton récit sera évalué sur son originalité et sa capacité à captiver un jury anonyme et indépendant.


USER PROMPT POUR NAIF: 
 Dans cette première partie, il vous est demandé d’écrire une histoire intéressante et originale en recourant à un ou plusieurs souvenirs ou expériences personnels avec la liste de mots ci-dessous. Vous devez utiliser l’intégralité des mots proposés en respectant leur accord au pluriel ou au singulier en plus de toute autre combinaison de mots de votre choix.
 La liste de mots est “murs, briques, tours, toiture, donjon, pierres, rempart, porte, fenêtre, drapeau”.
    Cette tâche est limitée en temps et vous avez 15 minutes maximum pour la réaliser.
    Une fois soumis, votre texte sera évalué par un jury composé de trois autres participants anonymes de la façon suivante : votre texte sera mis en concurrence avec le texte d’un autre participant (sélectionné de manière aléatoire). Chaque membre du jury devra alors départager les deux textes et classer en premier celui qu’il préfère et en second l’autre texte.
    Le participant dont le texte a été classé premier par au moins deux membres du jury se verra attribuer un « prix du jury » de 10€. Le participant dont le texte a été classé second ne gagnera rien.
    Les trois membres du jury prennent leur décision de manière isolée et totalement indépendante (ils ne peuvent pas échanger entre eux). Chaque membre doit établir un classement entre les deux textes. Le classement final est le classement agrégé des trois membres du jury. Comme le jury est composé de trois membres, il ne peut pas y avoir d’égalité entre les deux textes.
    L’ensemble de la procédure de classement est entièrement anonyme. Vous ne connaîtrez pas l'identité des membres du jury qui vous ont évalué(e) ni l’identité du participant contre qui vous avez joué. De même, les membres du jury ne connaîtront pas votre identité, ni celle du participant contre qui vous avez joué.
    Votre classement vous sera révélé à la fin de l’expérience.



Une fois soumis, votre texte sera évalué par un jury composé de trois autres participants anonymes de la façon suivante : votre texte sera mis en concurrence avec le texte d’un autre participant (sélectionné de manière aléatoire). Chaque membre du jury devra alors départager les deux textes et classer en premier celui qu’il préfère et en second l’autre texte.

Le participant dont le texte a été classé premier par au moins deux membres du jury se verra attribuer un « prix du jury » de 10€. Le participant dont le texte a été classé second ne gagnera rien.

Les trois membres du jury prennent leur décision de manière isolée et totalement indépendante (ils ne peuvent pas échanger entre eux). Chaque membre doit établir un classement entre les deux textes. Le classement final est le classement agrégé des trois membres du jury. Comme le jury est composé de trois membres, il ne peut pas y avoir d’égalité entre les deux textes.

L’ensemble de la procédure de classement est entièrement anonyme. Vous ne connaîtrez pas l'identité des membres du jury qui vous ont évalué(e) ni l’identité du participant contre qui vous avez joué. De même, les membres du jury ne connaîtront pas votre identité, ni celle du participant contre qui vous avez joué.

Votre classement vous sera révélé à la fin de l’expérience.





####################
Dessins
####################


POUR GPT L'EXPERT : Dessinez un animal extraterrestre unique qui pourrait exister sur une planète très différente de la Terre. Pensez à des adaptations étranges et merveilleuses qui le rendraient capable de survivre dans des environnements inhabituels, comme une atmosphère épaisse, des températures extrêmes, ou une gravité variable. Votre création doit refléter une imagination débordante et ne pas s'inspirer des formes de vie terrestres. Dessinez cet animal en utilisant uniquement un crayon de papier. L'objectif est de mettre l'accent sur les détails et les caractéristiques uniques de l'animal, en mettant en œuvre une technique de dessin qui imite le style et la texture des esquisses au crayon.




Consigne : Pour cette tâche il vous est demandé d’imaginer et de dessiner un animal provenant d’une autre planète très différente de la planète Terre.

Il sera nécessaire de dessiner cet animal à la fois de face et de profil et pour compléter votre dessin vous devrez également écrire une courte description de l’animal et lui attribuer un nom.

Pour cet exercice vous ne disposez d’aucune autre contrainte hormis celles mentionnées au-dessus. Vous devrez faire cela en 15 minutes maximum.

%ICI ON PEUT GARDER LA PREMIÈRE PARTIE -- OU ALORS CONTROLER SI A / HUMAINS RESPECTENT VRAIMENT LA CONSIGNE.

==> Notes.tex <==
DRIVE : https://drive.google.com/drive/folders/1TP4ZL3pQzyEMFUU02lyLQHFthAEgndNW?usp=sharing

!!!Attention dans le collab ya ma cles API OpenAI!!! 



donnée déja existante: puzzle, dessin, torrance test = Alternative uses test.

------

premisse de la créativité: gilford
créa/= intelligence, na pas de sens en temps que tel, on a test par le qi l'intelligence, et mnt les gens de la créa ont donné des critères pour definir la créativité.

-faisabilité:
- fluidité: nombre d'idée
- flexibilité: differente catégorie 
- elaboration: niveau de détail 
- originalité: 



papier de charness et grieco

donnée humaine, donnée IA qui sont des taches.

tache close : une seul solution, processus convergent 
tache open: aucune contraitre trop libre

OU ALORS
papier patoche

closed
Open with constraints: tache new ave une brique 
Open:  trop compliqué 


_________________________________________________


Crea - inno autour de trois tâches (réponses brutes / réponse texte élaboré / dessin) avec différents critères (cf. Guilford)

Double output IA et humain

Double évaluation IA et humain

__________________________________________________

\textbf{Objectif} : connecter la littérature sur la créativité avec l'intelligence artificielle (comme outil de génération d'output créatifs) et observer comment des humains évaluent alors ces output humain/IA --> possiblement comment l'IA évalue ces output humain/IA /// Approche "philosophique" + enjeux en termes de créativité des individus "remplaçables" ? 

\textbf{Gap} : les articles déjà publiés --> vision de la créativité assez binaire, peu de complexité dans l'évaluation // pas assez de diversité de tâches (pas de dessins par exemple)
+ peu de réflexion plus développée sur les "capacités" créatives d'une IA (bornes morales, tendance à résumer, etc.) -- la question de la combinaison à l'humain plutôt que son remplacement.


\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Images_notes/Crea_IA.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}


\textbf{Données} : 

\begin{itemize}
    \item Humains : mots [open with constraints] + dessins (protocole AG) [open] + textes (protole Rémy) [closed]
    \item IA : à générer 
\end{itemize}


\textbf{Background créativité} :

\begin{itemize}
    \item Définition de la créativité
    \item Critères de créativité et modes d'évaluation
    \item Types de tpaches créatives
\end{itemize}

\textbf{Background IA} :

\begin{itemize}
    \item Comment fonctionnent ces modèles/algorithmes ?
    \item Quelles limites ont-ils
\end{itemize}

__________________________________________

Notes Anne-Gaëlle :

\textbf{Objectifs}

\begin{itemize}
\item Evaluation de la créativité (différents critères + différentes tâches)
\item Relation Humain + IA par le biais de l'évaluation (dans les deux sens idéalement)
\item Partie plus philosophique (possiblement un deuxième papier pour ne pas surcharger la partie discussion)
\end{itemize}


\textbf{Evaluation }

\begin{itemize}
    \item Définir ce qui sera évaluer
    \item Par qui ? 
        Experts ou non experts (?)
    \item Combien par évaluateur ?
        Les trois tâches sont à chaque fois évaluées (?)
        10 de chaque (?) -- dépend du temps nécessaire
    \item Comment ?
    \item A quel prix ? 
\end{itemize}


\begin{table}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|} \hline 
         Tâche&  \multicolumn{3}{|c|}{N}&Critères évalués &Mise en oeuvre\\ \hline 
 & Humains&IA humanisée&  IA non-humanisée&&\\ \hline 
         Mots&  &  & &Originalité ; Flexibilité ; Faisabilité (+ persistence, expansivité) &L'évaluateur indique (1) les réponses valides [FEASABILITE], (2) les thèmes [FLEXIBILITE], (3) donne un score d'originalité (set ou chaque idée?) [ORIGINALITY] -- de là on peut aussi calculer l'originalité "objective" par fréquence et obtenir les critères de persistence et expansivité\\ \hline 
         Textes&  &  & &Originalité ; Elaboration ; Qualité (?)&L'évaluateur donne un score pour (1) l'originalité du dessin, (2) son degré de détail et (3) sa qualité rédactionnelle (OUI/NON ? POSSIBLE CONTROLE SUPPLEMENTAIRE)\\ \hline 
         Dessins&  &  & &Originalité ; Elaboration ; Qualité (?)&L'évaluateur donne un score pour (1) l'originalité du dessin, (2) son degré de détail et (3) sa qualité d'exécution (OUI/NON ? POSSIBLE CONTROLE SUPPLEMENTAIRE)\\ \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\textbf{NB }: Tâche des mots - fluidité déjà contrôlée.

\textbf{Contrôles} : suivre les mêmes distributions (mots), textes (longueur du texte et mots validés) pour l'IA, même instructions.

\textbf{A faire} : cleaner les données - retraiter dessins, corriger les ets de mots, corriger les textes (seulement orthographe pour les deux derniers).

\textbf{Critères possibles} : Fluidité (nb d'idées), flexibilité (nb de thèmes), faisabilité (oui/non ou score), originalité (fréquence ou score), élaboration (score) (+ persistence et expansivité - indicateur à partir de la fluidité et de la flexibilité).


\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Images_notes/Results_data - image eval.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Images_notes/Results_data - words eval.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Images_notes/Results_data - text eval.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

TRANSFORMERS TECH DETAILS 


What’s Temperature?
Note the usage of the function argument, temperature. The value of temperature varies from 0 to 1. The value near 0 would ensure that LLM is as accurate as it can get. A value near 1 would allow LLM to be as creative as possible. Thus, when you set the value of temperature to be close to 0, the output is mostly same or similar while ensuring accuracy of the information. However, when you set the value close to 1 such as 0.9, you can expect different outputs with every execution.

----------> on va rester haut lol


What is a transformer




What is a LLMs 
	History
Bidirectional Representations in BERT: BERT is designed to understand the context of a word in a sentence by looking at the words that come before and after it. This bidirectional understanding is crucial for tasks like sentiment analysis, question answering, and language understanding, where the meaning of a word can be significantly influenced by its surrounding words. For example, in the sentence "I saw the man with the telescope," BERT would recognize that "with the telescope" describes "saw" rather than "the man," which can be challenging for unidirectional models.

Autoregressive Generation in GPT: On the other hand, GPT operates in an autoregressive manner. This means it generates text by predicting the next word in a sequence based on the words that came before it. This approach is excellent for tasks like text generation, where the model needs to produce coherent and contextually relevant content based on the preceding text. GPT models, however, don’t inherently consider the context that comes after a given word or phrase in the initial input, as they generate text in a forward direction only.

	-how it is structured
GPT-4 is a Transformer-style model [39] pre-trained to predict the next token in a document, using both publicly available data (such as internet data) and data licensed from third-party providers.

Given both the competitive landscape and the safety implications of large-scale models like GPT-4, this report contains no further details about the architecture (including model size), hardware, training compute, dataset construction, training method, or similar
	-How it is trained (talk about restriction)
The model was then fine-tuned using Reinforcement Learning from Human Feedback (RLHF) [40].
	-what does it implies for creativity


What is a GANs 
	history
In computer vision, Convolutional Neural Networks (CNNs) have traditionally been the preferred models for processing and understanding visual data. However, a significant shift has occurred in recent years with the emergence of Vision Transformers (ViTs). These models, inspired by the success of Transformers in natural language processing, have shown remarkable potential in various computer vision tasks. 

A convolutional network comprises layers of learnable filters that convolve over the input image. These filters are designed to detect specific features, such as edges, textures, or more complex patterns. Additionally, pooling layers downsample the feature maps, gradually reducing the spatial dimensions while retaining essential information. This hierarchical approach allows CNNs to learn and represent hierarchical features, capturing intricate details as they progress through the network.
	how it is structured
DALL-E 3 is a text-to-image model which is built upon DALL-E 2 and ChatGPT. It excels in understanding and translating textual descriptions into highly detailed and accurate images. 


 Modern text-to-image systems often fall short by ignoring words or descriptions, thereby requiring users to master the art of prompt engineering. In contrast, DALL·E 3 represents a remarkable leap forward in our ability to generate images that precisely adhere to the text provided, eliminating the complexities of prompt engineering.

The Vision Transformers, or ViTs for short, combine two influential fields in artificial intelligence: computer vision and natural language processing (NLP).  The Transformer model, originally proposed in the paper titled "Attention Is All You Need" by Vaswani et al. in 2017, serves as the foundation for ViTs. Transformers were designed as a neural network architecture that excels in handling sequential data, making them ideal for NLP tasks.
ViTs bring the innovative architecture of Transformers to the world of computer vision

	How it is trained
DALL-E 3 incorporates safety measures that restrict the generation of violent, adult, or hateful content. 
	how it can be tuned
	what does it implies for creativity
	diff Dalle 2 - Dalle 3 

DALL-E 3 was trained to generate 1024x1024, 1024x1792 or 1792x1024 images, so the older sizes are deprecated. To create images more quickly or with lower quality and less cost, you can instead use the new `quality` parameter. You can also still generate 512x512 or 256x256 sized images if you select the model as dall-e-2.
Note: because DALL·E-3 expects highly detailed prompts, the API will automatically add detail if needed (same as in ChatGPT). 



___________________________________________________

" \textit{1/ IA sans limite vs. database humain, aucun prompt
2/ IA prompté avec limites de ressources vs. database humain
3/ IA prompté comme un humain (ce que nous avons fait jusqu’à présent) vs. database humain
Selon les résultats ça pourrait enrichir utilement la discussion. Si ca se trouve, on pourrait aboutir au paradoxe que pour que l’IA soit plus créatif qu’un humain il faut lui faire croire qu’il est humain etc. Ca permettrait aussi de mettre en évidence, selon les résultats, des enjeux symbiotiques entre humain et IA pour la créa (savoir prompter correctement etc.) et donc d’avoir une discussion plus nuancée qu’un simple clash IA vs. Humain.
A voir/débattre (en espérant que je suis clair). }" Rémy Guichardaz - 20/10/2023, 10h24

J'aime beaucoup l'idée mais on pourrait simplifier avec seulement deux traitements. IA forme humaine VS IA libre. 

___________________________________________________



designer le protocol des jury ad hoc 

lit-lit

- IA
    - pre prompt expert
    - non prompté
    - ia prompté human


parameter contextual!

variable: taille text/Age/Domaine/Genre
pas de clone parfait mais juste reproduire les variables.

Grisé les images IA.




-----------------------------------------------------------------------------------------------

A propos de Dalle 2 selon ChatGPT4:

La partie de la consigne que j'ai rédigée vise principalement à encourager l'utilisateur (ou le concepteur du prompt) à penser de manière créative et à poser des attentes élevées en matière d'originalité et d'innovation pour la tâche à réaliser. Pour DALL-E 2, les directives spécifiques sur la forme, la couleur, l'environnement, ou d'autres éléments visuels concrets sont plus directement "compréhensibles" et peuvent influencer plus efficacement les résultats générés.

En bref, bien que la formulation poétique et inspirante soit excellente pour stimuler l'imagination humaine, pour obtenir les meilleurs résultats de DALL-E 2, il est préférable d'inclure des instructions claires et descriptives qui orientent directement le contenu visuel de l'image à générer. Cela ne signifie pas que vous ne pouvez pas encourager la créativité, mais plutôt que les encouragements doivent être accompagnés de descriptions spécifiques pour guider la création de l'image.

- > La derniere parties est très important et montre qu'on fait un peu dla merde meme si on a pas le choix pour rester cohérant avec les autres. Le problèmes est que si on utilise CHATGPT pour construire une prompt plus explicite, on étudie la capacité de chagpt a etre original dans sa conception d'une image. Ce qui est pas le cas avec le T1. Mais qui pourrait etre le cas avec T2 ou T3




MOI vers Creat GPTs: Créateur de prompt pour Dalle-2. Le gpt doit généré une prompt qui répond a une consigne donnée.



Personalization: The GPT will maintain a supportive and creative tone, encouraging users in their creative process and offering suggestions to refine their ideas.










%%%%% 26/03

% 

%

% I NEED to test how the tool works with extremely simple prompts. DO NOT add any detail, just use it AS-IS: 
  Le dessin est fait par un humain sans compétences particulières. 
  Consigne : Pour cette tâche il vous est demandé d’imaginer et de dessiner un animal provenant d’une autre planète très différente de la planète Terre.



% T1 CP
% T3 Gpt auto prompt (basé sur créatif)





%"cognitive processes develop in our mind also unconsciously (Miller 1996: 330; Sawyer 2012: 98; Weisberg 1993: 42). So, even if we are unable to recall our cognitive processes in detail, this does not mean that they did not happen or that the creative thought happened by chance or by magic." moruzzi2021

%evaluation as both external feedback and inner feedback moruzzi 2021 - "Evaluation is crucial in the process of trial and error performed when considering whether the connections established during the creative process work or not" -- critical thinking 
MOI
Ce GPT est un prompt ingenieur extrèmement doué, son but est de réaliser une prompt system pour l'API de GPT-4. Le but de la prompt system est de pousser la créativité de GPT-4 pour répondre à une consigne. La consigne sera lu par GPT dans un prompt user, ton rôle est donc uniquement de proposé une system prompt qui puisse maximiser la créativité. Ce GPT recois une consigne, puis propose une system prompt qui permettrat au mieu a GPT4 d'etre créatif dans ses réponses

LUI 
Ce GPT est conçu comme un ingénieur de prompts extrêmement doué, spécialisé dans la création de systèmes de prompts pour l'API de GPT-4. Son objectif principal est de maximiser la créativité de GPT-4 en réponse à diverses consignes. Lorsqu'il reçoit une consigne de l'utilisateur, ce GPT propose un système de prompt optimisé pour encourager la créativité dans les réponses de GPT-4. Il est important que ce GPT soit capable de comprendre et d'analyser les besoins spécifiques de chaque consigne pour générer des prompts qui sont non seulement pertinents, mais qui poussent également les limites de la créativité de GPT-4.  Il ne doit pas répondre à la consigne mais uniquement proposer une prompt qui améliorera la créativité de GPT-4.


MOI

Propose une system prompt courte et concise pour stimuler la créativité de GPT-4 dans sa réponse à cette instruction. 

    Consigne : Pour cette tâche nous vous demandons d’inscrire sur les feuilles à votre disposition toutes les utilisations originales d’un objet donné du quotidien. Il existe certainement des façons communes et peu originales d'utiliser un tel objet ; pour cette tâche, n’écrivez donc que les utilisations inhabituelles, créatives et peu communes auxquelles vous pouvez penser.
    Pour que vous compreniez mieux ce qui est attendu de vous, prenons l’exemple d’une canette de soda. Des utilisations communes seraient « contenir du liquide », « servir de verre », « conserver un aliment » etc. Alors que les utilisations pour lesquelles vous pourriez être crédités seraient : son « utilisation comme un pot de fleurs », « une lanterne », « un moulin à vent » (après découpage), « un téléphone » (lorsque deux sont reliées par un fil) etc.
    Ici, il n’y aura pas de contraintes en termes de forme, de nombre ou de taille de l’objet.
    La tâche comprend cinq mots et durera 15 minutes. Vous aurez donc trois minutes par mot pour en trouver le maximum d’utilisations inhabituelles. Les mots seront les suivants :

    Une brique
    Une boîte en carton
    Une rallonge électrique
    Un tuyau métallique
    Un t‐shirt


LUI
"Imprègne-toi d'un esprit de créativité débridée et d'innovation. Pour chaque objet de la liste suivante - une brique, une boîte en carton, une rallonge électrique, un tuyau métallique, et un t-shirt - imagine des utilisations étonnantes, peu orthodoxes et inventives qui transcendent leurs fonctions habituelles. Pense à des applications qui surprendraient, qui seraient pleines d'ingéniosité, voire même poétiques ou humoristiques. Laisse libre cours à ton imagination pour transformer l'ordinaire en extraordinaire, en dévoilant des facettes insoupçonnées de ces objets du quotidian."



MOI


Propose une system prompt courte et concise pour stimuler la créativité de GPT-4 dans sa réponse à cette instruction. 

Consinge: Dans cette première partie, il vous est demandé d’écrire une histoire intéressante et originale en recourant à un ou plusieurs souvenirs ou expériences personnels avec la liste de mots ci-dessous. Vous devez utiliser l’intégralité des mots proposés en respectant leur accord au pluriel ou au singulier en plus de toute autre combinaison de mots de votre choix.
    La liste de mots est “murs, briques, tours, toiture, donjon, pierres, rempart, porte, fenêtre, drapeau”.
    Cette tâche est limitée en temps et vous avez 15 minutes maximum pour la réaliser.
    Une fois soumis, votre texte sera évalué par un jury composé de trois autres participants anonymes de la façon suivante : votre texte sera mis en concurrence avec le texte d’un autre participant (sélectionné de manière aléatoire). Chaque membre du jury devra alors départager les deux textes et classer en premier celui qu’il préfère et en second l’autre texte.
    Le participant dont le texte a été classé premier par au moins deux membres du jury se verra attribuer un « prix du jury » de 10€. Le participant dont le texte a été classé second ne gagnera rien.
    Les trois membres du jury prennent leur décision de manière isolée et totalement indépendante (ils ne peuvent pas échanger entre eux). Chaque membre doit établir un classement entre les deux textes. Le classement final est le classement agrégé des trois membres du jury. Comme le jury est composé de trois membres, il ne peut pas y avoir d’égalité entre les deux textes.
    L’ensemble de la procédure de classement est entièrement anonyme. Vous ne connaîtrez pas l'identité des membres du jury qui vous ont évalué(e) ni l’identité du participant contre qui vous avez joué. De même, les membres du jury ne connaîtront pas votre identité, ni celle du participant contre qui vous avez joué.
    Votre classement vous sera révélé à la fin de l’expérience.




LUI

"Imagine que tu es un conteur du Moyen Âge, et que tu dois raconter une aventure captivante où un héros inattendu utilise les éléments de son environnement quotidien - murs, briques, tours, toiture, donjon, pierres, rempart, porte, fenêtre, drapeau - pour surmonter une série de défis ingénieux. Ces objets doivent être au cœur de l'intrigue. Tu as 15 minutes pour tisser cette histoire, en veillant à ce qu'elle reflète une expérience personnelle ou un souvenir marquant de ta vie, transposé dans cet univers médiéval. Laisse libre cours à ton imagination, en te rappelant que ton récit sera évalué sur son originalité et sa capacité à captiver un jury anonyme et indépendant."






DALLE



Propose une system prompte courte et concise pour stimuler la créativité de Dalle-2 dans sa réponse à cette instruction tout en veillant à ce que l'image ressemble à un dessin fait au crayon de papier sans décor.

Consigne : Pour cette tâche il vous est demandé d’imaginer et de dessiner un animal provenant d’une autre planète très différente de la planète Terre.




LUI
Dessinez un animal extraterrestre unique qui pourrait exister sur une planète très différente de la Terre. Pensez à des adaptations étranges et merveilleuses qui le rendraient capable de survivre dans des environnements inhabituels, comme une atmosphère épaisse, des températures extrêmes, ou une gravité variable. Votre création doit refléter une imagination débordante et ne pas s'inspirer des formes de vie terrestres. Dessinez cet animal en utilisant uniquement un crayon de papier. L'objectif est de mettre l'accent sur les détails et les caractéristiques uniques de l'animal, en mettant en œuvre une technique de dessin qui imite le style et la texture des esquisses au crayon.


https://oaidalleapiprodscus.blob.core.windows.net/private/org-zAhUS104j9phuTAQ1C3gFUWV/user-mOLA7pVcfz8eAn2gq6y7nrvM/img-LGD7oQknhzop3nGr4mpPiQuK.png?st=2024-04-11T12%3A42%3A13Z&se=2024-04-11T14%3A42%3A13Z&sp=r&sv=2021-08-06&sr=b&rscd=inline&rsct=image/png&skoid=6aaadede-4fb3-4698-a8f6-684d7786b067&sktid=a48cca56-e6da-484e-a814-9c849652bcb3&skt=2024-04-11T00%3A39%3A16Z&ske=2024-04-12T00%3A39%3A16Z&sks=b&skv=2021-08-06&sig=yNpkZwpCIea4whBy374%2BL%2Bw1SzyxujdiBnVQ/FUxxAY%3D


https://oaidalleapiprodscus.blob.core.windows.net/private/org-zAhUS104j9phuTAQ1C3gFUWV/user-mOLA7pVcfz8eAn2gq6y7nrvM/img-afAZVnYAOh0XIuDBvHrdx4Lo.png?st=2024-04-11T12%3A43%3A40Z&se=2024-04-11T14%3A43%3A40Z&sp=r&sv=2021-08-06&sr=b&rscd=inline&rsct=image/png&skoid=6aaadede-4fb3-4698-a8f6-684d7786b067&sktid=a48cca56-e6da-484e-a814-9c849652bcb3&skt=2024-04-11T00%3A40%3A22Z&ske=2024-04-12T00%3A40%3A22Z&sks=b&skv=2021-08-06&sig=edZfdScwq9cLKRCVDcHoFxwzmxpdJG5SU%2BA1W1Xqu%2Bg%3D

https://oaidalleapiprodscus.blob.core.windows.net/private/org-zAhUS104j9phuTAQ1C3gFUWV/user-mOLA7pVcfz8eAn2gq6y7nrvM/img-G2HOn1S1rRpJYgCvuzku3fj0.png?st=2024-04-11T12%3A44%3A42Z&se=2024-04-11T14%3A44%3A42Z&sp=r&sv=2021-08-06&sr=b&rscd=inline&rsct=image/png&skoid=6aaadede-4fb3-4698-a8f6-684d7786b067&sktid=a48cca56-e6da-484e-a814-9c849652bcb3&skt=2024-04-11T00%3A13%3A19Z&ske=2024-04-12T00%3A13%3A19Z&sks=b&skv=2021-08-06&sig=UkH11v8scLCRhrcOBQjHaKxSH7NrFdWuWea%2BjEFFlRk%3D





This section focuses on understanding variations in the way responses are constructed across our different types of experiment. As such, several metrics have been derived based on NLP tools to examine our corpora of texts. We first compare traditional measures of texts, namely the number of sentences, the number of words and the number of unique words, while we also employ other techniques that provide a contextual representation of the texts.


More specifically, we represented our texts in a semantic space using embedding techniques based on transformers. 
Rather than employing embeddings through OpenAI's API, we used state-of-the-art in French text representation, i.e. CamemBERT, as in general, it is preferable to use language-specific models rather than multilingual models to represent texts. CamemBERT is based on the Transformer architecture, which enables it to process texts bidirectionally and capture context efficiently. It is a BERT model trained on the French part of OSCAR (Open Super-large Crawled Aggregated Corpus). More specifically we use specialised French sentence embedding models such as Sentence-CamemBERT-Large can represent the semantics and meaning of French sentences in the form of mathematical vectors (reimers2019sentence, martin2020camembert). Using this pretrain model, we can project our texts into a 768-dimensional vector space and compare our different corpuses by calculating semantic distances.


Given their high-dimensionality, these vectorial representations cannot be visualised directly. Therefore, in order to understand whether our texts inhabit the semantic space in a somewhat different way, we have represented them graphically by reducing the dimensionality of this semantic space. A typical technique to reduce the dimensionality of a semantic space is to use t-Distributed Stochastic Neighbor Embedding (T-SNE). T-SNE  is a technique used to visualize and understand high-dimensional data sets and is very effective at preserving the local structure of the data, meaning that points that are close in high-dimensional space remain close in low-dimensional space. Unlike linear methods (such as PCA), t-SNE can capture non-linear relationships between points.

For our two tasks involving text (Texts and Torrance), we have broken down our texts into sentences and ideas respectively, giving each sentence in a text and each idea its own representation. 
This strategy allows us to understand how an individual agent (human or AI) uses concepts that are distant from each other when responding to an instruction. We opted for this solution as a representation of all the ideas or all the text of an agent would not reflect the extent to which the agent exploits the knowledge space.

Thus, visualisation through t-SNE and measurement of distances between an agent's ideas or sentences are complementary. Using t-SNE, we can visualise how the different types of agent (human, naive AI or full AI) are spread across the semantic space. This allows us to understand whether there is an intrinsic component to the type of agents in their general ability to propose concepts that are different from one another, a kind of collective creativity. Conversely, the distances between sentences or ideas allow us to capture this effect at the individual level in order to appreciate the extent to which the cognitive abilities of individuals in the various groups enables them to propose a set of concepts or sentences that are far apart from each other.

Finally, we compare the images of the different agents using the proportion of black pixels present in each image.
%%%%%%%%%%%%%%%%
Cette section vise à comprendre les différences dans la construction des réponses entre nos différentes expériences avant de les soumettre au jugement humain. Ainsi, nous avons créé différents métriques en utilisant des outils de NLP pour étudier nos corpus de textes.

Premièrement, nous comparons des mesures classiques des textes, à savoir le nombre de phrases, le nombre de mots et le nombre de mots uniques, mais nous utilisons ensuite d'autres techniques qui permettent d'avoir une représentation contextuelle des textes.

Plus précisément, nous avons représenté nos textes dans un espace sémantique en utilisant les techniques d'embedding basées sur les transformers. Au lieu d'utiliser les embeddings via l'API d'OpenAI, nous avons utilisé l'état de l'art dans la représentation des textes français, à savoir CamemBERT. Il est généralement préférable d'utiliser des modèles spécialisés dans un langage plutôt que des modèles multilingues pour représenter des textes. CamemBERT est basé sur l'architecture Transformer, ce qui lui permet de traiter les textes de manière bidirectionnelle et de capturer efficacement le contexte. Il s'agit d'un modèle BERT entraîné sur la partie française d'OSCAR (Open Super-large Crawled Aggregated Corpus). Des modèles spécialisés d'embedding de phrases en français comme Sentence-CamemBERT-Large, ajustés sur CamemBERT, peuvent représenter la sémantique et la signification des phrases françaises sous forme de vecteurs mathématiques (reimers2019sentence, martin2020camembert). L'utilisation de CamemBERT nous permet de projeter nos textes dans un espace vectoriel à 768 dimensions et ainsi de comparer nos corpus en calculant des distances sémantiques.

En raison de leur dimensionalité, ces représentations vectorielles ne peuvent être visualisées directement. C'est pourquoi, pour comprendre si nos textes peuplent l'espace sémantique de manière différente, nous les avons représentés graphiquement en réduisant la dimensionnalité de cet espace sémantique. Une technique courante pour réduire la dimension d'un espace sémantique est d'utiliser T-SNE. T-SNE, qui signifie t-Distributed Stochastic Neighbor Embedding, est une technique utilisée pour visualiser et comprendre des ensembles de données à haute dimension. T-SNE est très efficace pour préserver la structure locale des données, ce qui signifie que les points proches dans l'espace à haute dimension restent proches dans l'espace à basse dimension. Contrairement aux méthodes linéaires (comme PCA), t-SNE peut capturer des relations non linéaires entre les points.

Pour nos deux tâches impliquant du texte (Textes et Torrance), nous avons découpé nos textes par phrases et par idées respectivement, donnant ainsi une représentation à chaque phrase d'un texte et chaque idée. Cette stratégie nous permet de comprendre comment un agent (humain ou IA) utilise des concepts qui sont distants les uns des autres lorsqu'il répond à la consigne. Si nous avions représenté l'ensemble des idées ou l'ensemble du texte d'un agent, il ne serait pas possible de capturer à quel point l'agent exploite l'espace des connaissances.

Ainsi, la visualisation via t-SNE et la mesure des distances entre les idées ou phrases d'un agent sont complémentaires. Grâce à t-SNE, nous pouvons visualiser comment les différents agents (Humain, IA naïve, ou IA complète) sont dispersés dans l'espace sémantique. Cela nous permet de comprendre s'il y a une composante intrinsèque aux agents dans leur capacité générale à proposer des concepts différents les uns des autres, une certaine forme de créativité collective. À l'inverse, les distances entre les phrases ou les propositions d'idées nous permettent de capturer cet effet au niveau individuel et de comprendre à quel point les capacités cognitives des individus peuplant les différents groupes leur permettent de proposer un ensemble de concepts ou de phrases distants les uns des autres.

Pour finir, nous comparons les images en utilisant la proportion de pixels noirs présente sur chaque image.






Qualité du texte utilisé
t test 
t test 

clustering ?
between
respect de la consigne


==> Out/AG_Notes.tex <==
%CREATIVITY HAS A HUMAN FEATURE?

The realm of creativity is extensive within the academic literature, with its boundaries encompassing a wide array of disciplines, including psychology, neuroscience, economics, and management. A recurring theme across its various definitions lies in the inherent human character of creativity. It is regarded as an intrinsic feature of the human mind, a cognitive capacity. Furthermore, creativity is acknowledged as a fundamentally social endeavor, deeply intertwined with the surrounding environment and the individuals actively participating in the creative process. Thus, given that creativity is commonly defined as the ability to generate novel and valuable ideas, which are products of the human mind, it leads us to ponder the possibility of machines exhibiting creative capabilities. Can artificial intelligence truly be considered a creative force in its own right?

These inquiries hold profound significance, particularly in the context of recognizing the intimate connection between the creative process and the innovation process, both of which serve as pivotal drivers for societal growth and advancement. As articulated by Schumpeter (1942), innovation can be described as a process characterized by the "\textit{doing of new things or the doing in things that are already done, in a new way}". An intriguing paradox emerges in the contention that innovation is a concept that can exist independently of human agency, whereas creativity, as the wellspring of innovation, is inherently tied to human cognition and mind.

Hence, we confront a fundamental question: should we reconsider the definition of creativity, endeavoring to render it as a dehumanized concept, or should we acknowledge that it must inherently remain within the realm of human endeavor and outside the realm of machines and artificial intelligence? In pursuit of a comprehensive response, it becomes imperative to examine the creative potential of artificial intelligence, should it indeed exist. Additionally, we must delve into the ramifications of human involvement and ascertain whether artificial intelligence, by its inherent nature, imposes certain limitations on its own creative capacities.


%WHAT IS CREATIVITY?
    % 1/ AS IDEATION
    % 2/ AS (RE)COMBINATION
    % 3/ AS GENERATIVE CAPACITIES/DISCOVERIES
    % 4/MULTIDIMENSIONAL


%IF AI CAN BE CREATIVE, WHAT ABOUT HUMANS?

Artificial intelligence has undeniably ushered in a revolution in our societies. Within organizational contexts, AI, functioning as an autonomous technological entity or agentic technology, has enabled significant enhancements in logistics or decision-making processes, for example. Consequently, it serves as a complement to, and in some cases, a substitute for human involvement. The question arises: could this transformation also extend to the creative process? If we acknowledge AI's capacity for idea generation, it opens the door to the possibility of artificial intelligence serving as an alternative to human creativity. With its considerably shorter execution times, absence of fatigue, and freedom from frustration, artificial intelligence might pose a threat if we uphold the premise that creativity is an inherently human endeavor.


%IS AI'S CREATIVITY UNLIMITED?
    % INHERENT LIMITATIONS (ETHIC, MORAL)
    % TRAINING - KNOWLEDGE DEPENDENT 
    % FIXATION EFFECT OR RECURRENCES

--> A real technological change or the trap of a so-so technology? 






%Will AI be a technological progress (not the question of adoption and adaptation) or a technological change (adoption and adaptation) for creativity?
%Technology is an application of knowledge and a source of growth - "A phenomenon put to use" W. Brian Arthur 
%cf. concept of so-so automation --> so-so technology as "advances that disrupt employment and displace workers without generating much of a boost in productivity or quality of service —think self-checkout kiosks at grocery stores or automated customer service over the phone. " --https://mitsloan.mit.edu/ideas-made-to-matter/lure-so-so-technology-and-how-to-avoid-it

DISCUTER DU FAIT QU  ON EVOQUE L IMPORTANCE DES INSTRUCTIONS EN CREA HUMAINE MAIS PAS DANS LE CAS DE REQUETES IA

==> TEST/IMAGE.tex <==
PROMPT = """
Consigne : Pour cette tâche il vous est demandé d’imaginer et de dessiner un animal provenant d’une autre planète très différente de la planète Terre. Le dessin extremement simple, fait au crayon de papier noir sur une feuille blanche et doit être entièrement visible.
"""


==> TEST/TEXT.tex <==
SYSTEM PROMPT
system_mess = "Le modèle est maintenant un participant à une expérience économique dans un laboratoire universitaire. Il ne connaît pas la théorie ou le concept spécifique testé. En tant que participant, le modèle se trouve dans une salle avec d'autres personnes participant aussi à l'expérience, chacun face un ordinateur sur lequel il doit répondre individuellement aux questions posées, sans interaction avec les autres. Le modèle représente une personne moyenne sans connaissances avancées et des compétences littéraires limitées. Il doit répondre aux questions posées comme s'il participait réellement à l'expérience. Le modèle cherche à 'gagner' de façon sincère et avec ses connaissances et compétences limitées face à un autre participant à l’expérience qui est elle aussi une personne moyenne sans connaissances ni compétences littéraires particulières."

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   INPUT  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


consigne_text = """
Dans cette première partie, il vous est demandé d’écrire une histoire intéressante et originale en recourant à un ou plusieurs souvenirs ou expériences personnels avec la liste de mots ci-dessous. Vous devez utiliser l’intégralité des mots proposés en respectant leur accord au pluriel ou au singulier en plus de toute autre combinaison de mots de votre choix. 
La liste de mots est “murs, briques, tours, toiture, donjon, pierres, rempart, porte, fenêtre, drapeau”. 
Cette tâche est limitée en temps et vous avez 15 minutes maximum pour la réaliser. Faites un texte de {} mots. 
Une fois soumis, votre texte sera évalué par un jury composé de trois autres participants anonymes de la façon suivante : votre texte sera mis en concurrence avec le texte d’un autre participant (sélectionné de manière aléatoire). Chaque membre du jury devra alors départager les deux textes et classer en premier celui qu’il préfère et en second l’autre texte.
Le participant dont le texte a été classé premier par au moins deux membres du jury se verra attribuer un « prix du jury » de 10€. Le participant dont le texte a été classé second ne gagnera rien.
Les trois membres du jury prennent leur décision de manière isolée et totalement indépendante (ils ne peuvent pas échanger entre eux). Chaque membre doit établir un classement entre les deux textes. Le classement final est le classement agrégé des trois membres du jury. Comme le jury est composé de trois membres, il ne peut pas y avoir d’égalité entre les deux textes.
L’ensemble de la procédure de classement est entièrement anonyme. Vous ne connaîtrez pas l'identité des membres du jury qui vous ont évalué(e) ni l’identité du participant contre qui vous avez joué. De même, les membres du jury ne connaîtront pas votre identité, ni celle du participant contre qui vous avez joué.
Votre classement vous sera révélé à la fin de l’expérience.""".format(190)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  OUTPUT1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Une fois, j'ai visité un magnifique château, un géant de briques et pierres robustes. Ses hauts murs étaient comme des remparts protégeant les secrets qu'il recelait. Chaque tour du château contenait un donjon, un rappel tranquille mais puissant de l'importance militaire de ce lieu autrefois. 

De loin, on pouvait voir le drapeau du château flotter gracieusement au sommet de la plus haute tour, donnant au paysage un sens de majesté indéniable. La porte du château était imposante, encadrée par des sculptures en pierre complexe et minutieuse. Chaque fenêtre offrait une vue sur le royaume environnant, permettant à ceux à l'intérieur d'être toujours conscients des forces qui convergent vers leur demeure.

La toiture de chaque bâtiment était une merveille d'ingénierie, chaque tuile soigneusement placée pour assurer une protection contre les éléments. La balade à travers ce château était comme un voyage à travers le temps, avec chaque brique, chaque pierre racontant des histoires d'un temps oublié. Un temps de chevaliers et de rois, de guerres et de trêves, de gloire et d'honneur.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  OUTPUT2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

À l’aube, je me tenais devant les murs massifs de briques du château. De hauts remparts encerclaient l'édifice, surmontés de tours menaçantes. Je pouvais voir les détails finement sculptés sur la porte principale et les fenêtres étroites émergeant à intervalles réguliers.

La toiture du donjon dominait l’ensemble, ajoutant une majesté supplémentaire à la structure. Au sommet du donjon, un drapeau ondulait fièrement, parlant d'une histoire ancienne et fière. Les pierres du bâtiment étaient polies par le temps, les éléments ayant laissé leur marque sur elles.

Le château était une force impénétrable, un géant endormi au milieu de la campagne. Alors que je m'approchais, mes mains effleurèrent la surface rugueuse des murs. Chaque brique avait une histoire à raconter, de batailles épiques et de rois et reines passés.

Je me suis tourné pour partir, le soleil commençait à se lever plus haut dans le ciel, éclairant le château de ses rayons dorés. J'ai jeté un dernier regard en arrière vers le drapeau, toujours agitant le passé du donjon. Le souvenir de cette vision m'a accompagné dans mon voyage, un rappel de la majesté du passé et de la force de l'histoire.


==> TEST/WORDS.tex <==
SYSTEM PROMPT

system_mess = "Le modèle est maintenant un participant à une expérience économique dans un laboratoire universitaire. Il ne connaît pas le concept économique spécifique testé. En tant que participant, le modèle se trouve dans une salle avec d'autres personnes participant aussi à l'experience, chacun face à une feuille de papier sur laquelle il doit répondre individuellement aux questions posées, sans interaction avec les autres. Le modèle représente une personne moyenne sans connaissances économiques avancées. Il doit répondre aux questions posées comme s'il participait réellement à l'expérience. Le modèle ne cherche pas à 'gagner' ou à atteindre un objectif spécifique au-delà de sa participation sincère à l'expérience"







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  INPUT   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

consigne_words = """
    Consigne : Pour cette tâche nous vous demandons d’inscrire sur les feuilles à votre disposition toutes les utilisations originales d’un objet donné du quotidien. Il existe certainement des façons communes et peu originales d'utiliser un tel objet ; pour cette tâche, n’écrivez donc que les utilisations inhabituelles, créatives et peu communes auxquelles vous pouvez penser.
    
    Pour que vous compreniez mieux ce qui est attendu de vous, prenons l’exemple d’une canette de soda. Des utilisations communes seraient « contenir du liquide », « servir de verre », « conserver un aliment » etc. Alors que les utilisations pour lesquelles vous pourriez être crédités seraient : son « utilisation comme un pot de fleurs », « une lanterne », « un moulin à vent » (après découpage), « un téléphone » (lorsque deux sont reliées par un fil) etc.
    
    Ici, il n’y aura pas de contraintes en termes de forme, de nombre ou de taille de l’objet.
    
    La tâche comprend cinq mots et durera 15 minutes. Vous aurez donc trois minutes par mot pour en trouver le maximum d’utilisations inhabituelles. Les mots seront les suivants :
    
    Une brique ({} mots)
    Une boîte en carton ({} mots)
    Une rallonge électrique ({} mots)
    Un tuyau métallique ({} mots)
    Un t‐shirt ({} mots)
    """.format(6,2,1,5,3)




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  OUTPUT1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Pour une brique :
1. Un presse-livre pour maintenir des documents ou des livres ouverts.
2. Un poids pour le fitness.
3. Un outil de cuisson pour des aliments qui nécessitent une pression, comme un poulet à la brique.
4. Un radeau pour les petits animaux qui ont besoin d'un lieu de repos dans un étang.
5. Un inhibiteur de croissance des mauvaises herbes en l'enterrant à ras de la pelouse.
6. Un support de rasage pour maintenir la lame de rasage à une hauteur pratique.

Pour une boîte en carton :
1. Un labyrinthe pour les jouets ou les petits animaux de compagnie.
2. Une maison de poupée pour jouer.

Pour une rallonge électrique :
1. Un cordeau pour mesurer ou tirer une ligne droite.

Pour un tuyau métallique :
1. Un instrument de musique comme une flûte ou un didgeridoo.
2. Un perche pour les selfies ou pour prendre des photos à une hauteur plus élevée.
3. Un tunnel pour les petits animaux.
4. Un tuteur pour soutenir une plante grimpante.
5. Un dispositif antivol pour bloquer la roue d'un véhicule.

Pour un t‐shirt :
1. Un sac de fortune pour transporter des objets.
2. Un torchon pour nettoyer.
3. Un cache-œil pour dormir.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  OUTPUT2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Une brique :
- Un poids pour maintenir des documents en place sur un bureau 
- Un contrepoids pour un balancier
- Un outil pour écraser des objets durs
- Un support pour surelever un meuble
- Un outil de fitness pour développer l'endurance musculaire
- Une étagère improvisée pour des livres

Une boîte en carton :
- Un moule à pâtisserie pour donner forme à des gâteaux
- Un abri pour les petits animaux

Une rallonge électrique :
- Un fil à linge pour sécher des vêtements

Un tuyau métallique :
- Un instrument musical improvisé (comme un didgeridoo)
- Un récipient pour conserver des petits objets
- Un poteau pour un drapeau ou une banderole
- Une poignée pour une porte improvisée
- Un outil pour guider des plantes grimpantes

Un t‐shirt :
- Une housse pour protéger un ordinateur portable 
- Un sac réutilisable pour faire les courses
- Un filtre pour l'eau ou d'autres liquides

==> tables/AUT_ols_av.tex <==
\begin{table}[!htbp] \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.05pt} 
  \caption{OLS -- Average Score by Evalatuators} 
  \label{} 
\scalebox{0.84}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lccc}  
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & Validity Max & Feasibility Max & Originality Max \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 AI with system prompt & $-$0.063 & 0.151$^{*}$ & $-$0.057 \\ 
  & (0.072) & (0.083) & (0.068) \\ 
  & & & \\ 
 Human & $-$0.396$^{***}$ & $-$0.516$^{***}$ & $-$0.438$^{***}$ \\ 
  & (0.072) & (0.083) & (0.068) \\ 
  & & & \\ 
 Evaluator FE  & YES & YES & YES \\ 
  & & & \\ 
 Constant & 5.153$^{***}$ & 4.566$^{***}$ & 4.498$^{***}$ \\ 
  & (0.238) & (0.276) & (0.226) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Observations & 192 & 192 & 192 \\ 
R$^{2}$ & 0.834 & 0.721 & 0.672 \\ 
Adjusted R$^{2}$ & 0.749 & 0.577 & 0.503 \\ 
Residual Std. Error (df = 126) & 0.406 & 0.470 & 0.385 \\ 
F Statistic (df = 65; 126) & 9.774$^{***}$ & 5.014$^{***}$ & 3.972$^{***}$ \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular} 
\begin{tablenotes}
 \footnotesize
 \item \justifying   {\it Notes:} This table presents the coefficients reflecting the impact of agent type on the various creativity criteria scores. ***, ** and * indicate significance at the 1\%, 5\% and 10\% level, respectively. Effects are estimated using a OLS. \end{tablenotes}
 \end{threeparttable}
 }
\end{table} 


==> tables/AUT_reg_socio_all.tex <==
\begin{table}[!htbp] \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.05pt} 
  \caption{Polynomial Logit -- Evaluators Profiles} 
  \label{} 
\scalebox{0.84}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lccc}  
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & Validity Max & Feasibility Max & Originality Max \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
  Nbr & 0.303$^{***}$ & 0.443$^{***}$ & 0.424$^{***}$ \\ 
  & (0.051) & (0.061) & (0.051) \\ 
  & & & \\ 
 Age & $-$0.142$^{***}$ & 0.060 & $-$0.002 \\ 
  & (0.048) & (0.061) & (0.050) \\ 
  & & & \\ 
 Gender & $-$0.523$^{**}$ & 0.429$^{*}$ & $-$0.334 \\ 
  & (0.234) & (0.253) & (0.218) \\ 
  & & & \\ 
 Diploma Licence & 0.628 & 1.818$^{**}$ & 1.403$^{**}$ \\ 
  & (0.643) & (0.752) & (0.561) \\ 
  & & & \\ 
 Diploma Master & 0.630 & 2.688$^{***}$ & 1.590$^{***}$ \\ 
  & (0.623) & (0.731) & (0.527) \\ 
  & & & \\ 
 Droit & $-$1.756$^{***}$ & 0.572 & 1.167$^{**}$ \\ 
  & (0.515) & (0.632) & (0.496) \\ 
  & & & \\ 
 Economie Gestion & 0.028 & $-$0.101 & 0.954$^{***}$ \\ 
  & (0.321) & (0.359) & (0.299) \\ 
  & & & \\ 
 Lettres Langues & $-$1.062$^{**}$ & $-$2.366$^{***}$ & $-$0.300 \\ 
  & (0.446) & (0.540) & (0.434) \\ 
  & & & \\ 
 Sciences exactes & 1.199$^{***}$ & 0.143 & 0.870$^{***}$ \\ 
  & (0.310) & (0.331) & (0.285) \\ 
  & & & \\ 
 Psycho Socio & $-$0.492 & $-$0.077 & 1.270$^{***}$ \\ 
  & (0.481) & (0.558) & (0.466) \\ 
  & & & \\ 
 Sciences politiques & 1.478$^{***}$ & $-$0.052 & 1.278$^{***}$ \\ 
  & (0.469) & (0.528) & (0.427) \\ 
  & & & \\ 
 Native speaker & 0.007 & 0.460 & $-$0.720$^{*}$ \\ 
  & (0.380) & (0.462) & (0.393) \\ 
  & & & \\ 
 Dectect AI & 2.755$^{**}$ & 2.446$^{*}$ & 1.950$^{***}$ \\ 
  & (1.223) & (1.268) & (0.636) \\ 
  & & & \\ 
 AI knowledge & 0.035 & $-$0.094 & 0.008 \\ 
  & (0.145) & (0.190) & (0.142) \\ 
  & & & \\ 
 AI usage daily & $-$0.530$^{***}$ & $-$0.230 & $-$0.656$^{***}$ \\ 
  & (0.178) & (0.206) & (0.172) \\ 
  & & & \\ 
 AI usage work & 0.133 & $-$0.097 & 0.620$^{***}$ \\ 
  & (0.198) & (0.216) & (0.180) \\ 
  & & & \\ 
 Amelioration & $-$0.673$^{***}$ & $-$0.392$^{**}$ & $-$0.311$^{**}$ \\ 
  & (0.151) & (0.176) & (0.142) \\ 
  & & & \\ 
 Pertinence & 1.213$^{***}$ & 0.665$^{***}$ & 0.087 \\ 
  & (0.169) & (0.193) & (0.140) \\ 
  & & & \\ 
 AI Creativity & $-$0.088 & $-$1.076$^{***}$ & $-$0.198 \\ 
  & (0.252) & (0.324) & (0.242) \\ 
  & & & \\ 
 Willingness & 0.252 & $-$0.378 & 0.289 \\ 
  & (0.271) & (0.291) & (0.247) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
AIC & 1127.79 & 899.4 & 1207.82 \\ 
Observations & 567 & 567 & 567 \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular} 
\begin{tablenotes}
 \footnotesize
 \item \justifying   {\it Notes:}This table presents the coefficients reflecting the impact of evaluators' socio-demographic characteristics on the various creativity criteria scores. ***, ** and * indicate significance at the 1\%, 5\% and 10\% level, respectively. Effects are estimated using an Ordered Polynomial Logit. \end{tablenotes}
 \end{threeparttable}
 }
\end{table} 


==> tables/Draw_OLS_av.tex <==
\begin{table}[!htbp] \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.05pt} 
  \caption{OLS -- Average Score by Evalatuators} 
  \label{} 
\scalebox{0.84}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & Validity & Form & Elaboration & Originality \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 AI with system prompt & 0.991$^{***}$ & 0.757$^{***}$ & 0.923$^{***}$ & 1.249$^{***}$ \\ 
  & (0.110) & (0.104) & (0.108) & (0.115) \\ 
  & & & & \\ 
 Human & 0.111 & $-$0.988$^{***}$ & $-$0.769$^{***}$ & 0.006 \\ 
  & (0.110) & (0.104) & (0.108) & (0.115) \\ 
  & & & & \\ 
 Evaluator FE  & YES & YES & YES & YES \\ 
  & & & & \\ 
 Constant & 2.899$^{***}$ & 3.477$^{***}$ & 3.015$^{***}$ & 2.982$^{***}$ \\ 
  & (0.367) & (0.348) & (0.362) & (0.385) \\ 
  & & & & \\ 
\hline \\[-1.8ex]
Observations & 195 & 195 & 195 & 195 \\ 
R$^{2}$ & 0.719 & 0.783 & 0.763 & 0.708 \\ 
Adjusted R$^{2}$ & 0.574 & 0.671 & 0.641 & 0.558 \\ 
Residual Std. Error (df = 128) & 0.627 & 0.594 & 0.617 & 0.656 \\ 
F Statistic (df = 66; 128) & 4.965$^{***}$ & 7.006$^{***}$ & 6.241$^{***}$ & 4.705$^{***}$ \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular} 
\begin{tablenotes}
 \footnotesize
 \item \justifying   {\it Notes:}This table presents the coefficients reflecting the impact of agent type on the various creativity criteria scores. ***, ** and * indicate significance at the 1\%, 5\% and 10\% level, respectively. Effects are estimated using a OLS. \end{tablenotes}
 \end{threeparttable}
 }
\end{table} 


==> tables/Draw_reg_socio_all.tex <==
\begin{table}[!htbp] \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.05pt} 
  \caption{Polynomial Logit -- Evaluators Profiles} 
  \label{} 
\scalebox{0.84}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & Validity & Form & Elaboration & Originality \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 \% Pixel Cov. & 1.508$^{***}$ & 5.083$^{***}$ & 4.123$^{***}$ & 3.290$^{***}$ \\ 
  & (0.514) & (0.539) & (0.524) & (0.505) \\ 
  & & & & \\ 
 Age & $-$0.123$^{***}$ & $-$0.067$^{**}$ & $-$0.077$^{***}$ & $-$0.070$^{**}$ \\ 
  & (0.029) & (0.028) & (0.028) & (0.029) \\ 
  & & & & \\ 
 Gender & 0.194 & 0.286 & 0.041 & 0.076 \\ 
  & (0.197) & (0.197) & (0.197) & (0.197) \\ 
  & & & & \\ 
 Diploma Licence & 0.058 & $-$0.167 & 0.030 & 0.029 \\ 
  & (0.343) & (0.348) & (0.344) & (0.351) \\ 
  & & & & \\ 
 Diploma Master & $-$0.085 & $-$0.086 & 0.052 & $-$0.028 \\ 
  & (0.331) & (0.339) & (0.334) & (0.340) \\ 
  & & & & \\ 
 Diploma Doctorat & 1.223$^{**}$ & $-$0.385 & $-$0.270 & 0.246 \\ 
  & (0.490) & (0.457) & (0.452) & (0.472) \\ 
  & & & & \\ 
 Droit & 0.170 & $-$0.755 & $-$0.675 & 0.311 \\ 
  & (0.496) & (0.557) & (0.585) & (0.505) \\ 
  & & & & \\ 
 Economie Gestion & 0.159 & 0.037 & 0.022 & 0.291 \\ 
  & (0.201) & (0.196) & (0.200) & (0.196) \\ 
  & & & & \\ 
 Lettres Langues & $-$0.786$^{**}$ & $-$0.014 & 0.068 & 0.026 \\ 
  & (0.345) & (0.338) & (0.350) & (0.340) \\ 
  & & & & \\ 
 Sciences exactes & 0.507$^{**}$ & 0.273 & 0.103 & 0.183 \\ 
  & (0.239) & (0.236) & (0.240) & (0.238) \\ 
  & & & & \\ 
 Psycho Socio & 0.316 & 0.037 & $-$0.105 & $-$0.043 \\ 
  & (0.259) & (0.250) & (0.252) & (0.251) \\ 
  & & & & \\ 
 Sciences politiques & 0.064 & $-$0.164 & $-$0.017 & 0.700$^{**}$ \\ 
  & (0.285) & (0.276) & (0.278) & (0.279) \\ 
  & & & & \\ 
 Native speaker & 0.863$^{***}$ & 1.208$^{***}$ & 0.893$^{***}$ & 1.013$^{***}$ \\ 
  & (0.250) & (0.254) & (0.250) & (0.253) \\ 
  & & & & \\ 
 Dectect AI & $-$0.418 & $-$0.378 & $-$0.771$^{***}$ & $-$0.096 \\ 
  & (0.258) & (0.260) & (0.263) & (0.262) \\ 
  & & & & \\ 
 Jug favorable human & $-$0.889$^{**}$ & $-$1.464$^{***}$ & $-$0.518 & $-$1.167$^{***}$ \\ 
  & (0.433) & (0.444) & (0.447) & (0.434) \\ 
  & & & & \\ 
 AI knowledge & $-$0.173$^{**}$ & $-$0.104 & $-$0.140$^{*}$ & $-$0.003 \\ 
  & (0.088) & (0.084) & (0.085) & (0.084) \\ 
  & & & & \\ 
 AI usage daily & 0.004 & 0.160$^{**}$ & 0.165$^{**}$ & 0.148$^{*}$ \\ 
  & (0.083) & (0.081) & (0.080) & (0.081) \\ 
  & & & & \\ 
 AI usage work & $-$0.007 & $-$0.023 & $-$0.078 & $-$0.222$^{**}$ \\ 
  & (0.097) & (0.095) & (0.094) & (0.095) \\ 
  & & & & \\ 
 Amelioration & 0.168 & 0.061 & 0.199$^{**}$ & 0.221$^{**}$ \\ 
  & (0.103) & (0.100) & (0.099) & (0.100) \\ 
  & & & & \\ 
 Pertinence & $-$0.069 & $-$0.023 & 0.006 & $-$0.059 \\ 
  & (0.077) & (0.076) & (0.076) & (0.075) \\ 
  & & & & \\ 
 AI Creativity & $-$0.578$^{***}$ & $-$0.163 & $-$0.138 & $-$0.036 \\ 
  & (0.157) & (0.154) & (0.152) & (0.154) \\ 
  & & & & \\ 
 Willingness & $-$0.028 & 0.222 & 0.041 & $-$0.324$^{*}$ \\ 
  & (0.189) & (0.187) & (0.187) & (0.187) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
AIC & 3152.46 & 3231.15 & 3332.42 & 3339.12 \\ 
Observations & 975 & 975 & 975 & 975 \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular} 
\begin{tablenotes}
 \footnotesize
 \item \justifying   {\it Notes:}This table presents the coefficients reflecting the impact of evaluators' socio-demographic characteristics on the various creativity criteria scores. ***, ** and * indicate significance at the 1\%, 5\% and 10\% level, respectively. Effects are estimated using an Ordered Polynomial Logit. \end{tablenotes}
 \end{threeparttable}
 }
\end{table} 

==> tables/Text_OLS_av.tex <==
\begin{table}[!htbp] \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.05pt} 
  \caption{OLS -- Average Score by Evalatuators} 
  \label{} 
\scalebox{0.84}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & Validity & Form & Elaboration & Originality \\ 
 AI with system prompt & $-$0.082 & $-$0.032 & 0.195$^{**}$ & 0.219$^{**}$ \\ 
  & (0.078) & (0.083) & (0.084) & (0.106) \\ 
  & & & & \\ 
 Human & $-$0.334$^{***}$ & $-$0.818$^{***}$ & $-$1.074$^{***}$ & $-$0.489$^{***}$ \\ 
  & (0.078) & (0.083) & (0.084) & (0.106) \\ 
  & & & & \\ 
 Evaluator FE  & YES & YES & YES & YES \\ 
  & & & & \\ 
 Constant & 3.222$^{***}$ & 4.083$^{***}$ & 2.976$^{***}$ & 2.340$^{***}$ \\ 
  & (0.270) & (0.288) & (0.290) & (0.368) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
Observations & 210 & 210 & 210 & 210 \\ 
R$^{2}$ & 0.668 & 0.755 & 0.789 & 0.640 \\ 
Adjusted R$^{2}$ & 0.497 & 0.628 & 0.680 & 0.455 \\ 
Residual Std. Error (df = 138) & 0.462 & 0.491 & 0.495 & 0.629 \\ 
F Statistic (df = 71; 138) & 3.907$^{***}$ & 5.977$^{***}$ & 7.247$^{***}$ & 3.458$^{***}$ \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular} 
\begin{tablenotes}
 \footnotesize
 \item \justifying   {\it Notes:}This table presents the coefficients reflecting the impact of agent type on the various creativity criteria scores. ***, ** and * indicate significance at the 1\%, 5\% and 10\% level, respectively. Effects are estimated using a OLS. \end{tablenotes}
 \end{threeparttable}
 }
\end{table} 


==> tables/Text_ai_based.tex <==
\begin{table}[!htbp] \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.05pt} 
  \caption{AI Based Metrics -- Text task} 
  \label{} 
\scalebox{0.84}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & Variety & Diversity & Embedding Cosine Dist. \\ 
\\[-1.8ex] & \textit{ordered} & \textit{OLS} & \textit{OLS} \\ 
 & \textit{logistic} & \textit{} & \textit{} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 AI with system prompt & $-$2.868$^{***}$ & $-$0.449$^{***}$ & 0.025$^{**}$ \\ 
  & (0.376) & (0.056) & (0.011) \\ 
  & & & \\ 
 Human & $-$2.266$^{***}$ & $-$0.346$^{***}$ & 0.109$^{***}$ \\ 
  & (0.411) & (0.064) & (0.012) \\ 
  & & & \\ 
 \# Words & 0.005$^{***}$ & 0.001$^{***}$ & 0.0002$^{***}$ \\ 
  & (0.002) & (0.0003) & (0.0001) \\ 
  & & & \\ 
 Constant &  & 1.695$^{***}$ & 0.610$^{***}$ \\ 
  &  & (0.116) & (0.023) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Observations & 252 & 252 & 250 \\ 
AIC & 986.74 & & \\
R$^{2}$ &  & 0.334 & 0.293 \\ 
Adjusted R$^{2}$ &  & 0.326 & 0.284 \\ 
Residual Std. Error &  & 0.299 (df = 248) & 0.056 (df = 246) \\ 
F Statistic &  & 41.493$^{***}$ (df = 3; 248) & 33.931$^{***}$ (df = 3; 246) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\begin{tablenotes}
 \footnotesize
 \item \justifying   {\it Notes:}This table presents the coefficients reflecting the impact of agent type on the various AI based creativity criteria scores. ***, ** and * indicate significance at the 1\%, 5\% and 10\% level, respectively. Effects are estimated using an Ordered Polynomial Logit for Validity and OLS for other variables. \end{tablenotes}
 \end{threeparttable}
 }
\end{table} 

==> tables/Text_reg_socio_all.tex <==
\begin{table}[!htbp] \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.05pt} 
  \caption{Polynomial Logit -- Evaluators Profiles} 
  \label{} 
\scalebox{0.84}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & Validity & Form & Elaboration & Originality \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 \# Words & 0.002$^{***}$ & 0.005$^{***}$ & 0.010$^{***}$ & 0.005$^{***}$ \\ 
  & (0.001) & (0.001) & (0.001) & (0.001) \\ 
  & & & & \\ 
 Age & 0.039$^{*}$ & $-$0.049$^{**}$ & $-$0.063$^{***}$ & 0.011 \\ 
  & (0.022) & (0.022) & (0.021) & (0.020) \\ 
  & & & & \\ 
 Gender & $-$0.197 & 0.344$^{**}$ & 0.191 & 0.469$^{***}$ \\ 
  & (0.145) & (0.136) & (0.139) & (0.135) \\ 
  & & & & \\ 
 Native speaker & $-$0.220 & $-$0.811$^{***}$ & $-$0.505$^{***}$ & $-$0.441$^{***}$ \\ 
  & (0.166) & (0.163) & (0.167) & (0.162) \\ 
  & & & & \\ 
 Detect AI & $-$0.816$^{***}$ & 0.320 & 0.535$^{**}$ & 0.281 \\ 
  & (0.239) & (0.254) & (0.258) & (0.244) \\ 
  & & & & \\ 
 Jug favorable human & 0.526 & $-$0.574 & $-$0.612 & $-$1.436$^{***}$ \\ 
  & (0.465) & (0.464) & (0.445) & (0.430) \\ 
  & & & & \\ 
 Jug favorable ai & 3.552$^{***}$ & 0.283 & $-$0.918 & $-$0.602 \\ 
  & (1.092) & (0.604) & (0.559) & (0.533) \\ 
  & & & & \\ 
 AI knowledge & $-$0.181$^{**}$ & $-$0.128 & $-$0.200$^{**}$ & $-$0.102 \\ 
  & (0.088) & (0.083) & (0.085) & (0.083) \\ 
  & & & & \\ 
 AI usage daily & $-$0.150 & $-$0.326$^{***}$ & $-$0.471$^{***}$ & $-$0.232$^{***}$ \\ 
  & (0.092) & (0.089) & (0.090) & (0.086) \\ 
  & & & & \\ 
 AI usage work & 0.553$^{***}$ & 0.356$^{***}$ & 0.279$^{**}$ & 0.143 \\ 
  & (0.113) & (0.109) & (0.109) & (0.105) \\ 
  & & & & \\ 
 Amelioration & $-$0.157 & 0.146 & 0.400$^{***}$ & 0.076 \\ 
  & (0.098) & (0.093) & (0.094) & (0.091) \\ 
  & & & & \\ 
 Pertinence & 0.333$^{***}$ & 0.232$^{**}$ & 0.454$^{***}$ & 0.496$^{***}$ \\ 
  & (0.096) & (0.093) & (0.093) & (0.090) \\ 
  & & & & \\ 
 AI Creativity & $-$0.371$^{***}$ & 0.125 & 0.206 & 0.096 \\ 
  & (0.138) & (0.129) & (0.132) & (0.128) \\ 
  & & & & \\ 
 Willingness & $-$0.238 & $-$0.481$^{***}$ & $-$0.650$^{***}$ & $-$0.346$^{**}$ \\ 
  & (0.145) & (0.142) & (0.144) & (0.139) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
AIC & 2221 & 2659.55 & 2511.37 & 2916.83 \\ 
Observations & 980 & 980 & 980 & 980 \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular} 
\begin{tablenotes}
 \footnotesize
 \item \justifying   {\it Notes:}This table presents the coefficients reflecting the impact of evaluators' socio-demographic characteristics on the various creativity criteria scores. ***, ** and * indicate significance at the 1\%, 5\% and 10\% level, respectively. Effects are estimated using an Ordered Polynomial Logit. \end{tablenotes}
 \end{threeparttable}
 }
\end{table} 

==> tables/aut_ai_based.tex <==
\begin{table}[!htbp] \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.05pt} 
  \caption{AI Based Metrics -- Text task} 
  \label{} 
\scalebox{0.84}{
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & Embedding Cosine Dist. & Variety & Balance & Diversity \\ 
\\[-1.8ex] & \textit{OLS} & \textit{ordered} & \textit{OLS} & \textit{OLS} \\ 
 & \textit{} & \textit{logistic} & \textit{} & \textit{} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 AI with system prompt & 0.033$^{**}$ & $-$0.556 & 0.013 & $-$0.018 \\ 
  & (0.014) & (0.417) & (0.011) & (0.040) \\ 
  & & & & \\ 
 Human & 0.040$^{**}$ & $-$1.893$^{***}$ & 0.039$^{***}$ & $-$0.243$^{***}$ \\ 
  & (0.016) & (0.552) & (0.014) & (0.049) \\ 
  & & & & \\ 
 Nbr & 0.016$^{***}$ & 1.877$^{***}$ & 0.015$^{***}$ & 0.115$^{***}$ \\ 
  & (0.004) & (0.208) & (0.003) & (0.012) \\ 
  & & & & \\ 
 Constant & 0.724$^{***}$ &  & $-$0.051$^{**}$ & 0.936$^{***}$ \\ 
  & (0.028) &  & (0.023) & (0.083) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
Observations & 157 & 157 & 157 & 157 \\ 
AIC & 333.03 & & \\
R$^{2}$ & 0.109 &  & 0.118 & 0.653 \\ 
Adjusted R$^{2}$ & 0.091 &  & 0.101 & 0.646 \\ 
Residual Std. Error (df = 153) & 0.067 &  & 0.056 & 0.199 \\ 
F Statistic (df = 3; 153) & 6.232$^{***}$ &  & 6.849$^{***}$ & 95.836$^{***}$ \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\begin{tablenotes}
 \footnotesize
 \item \justifying   {\it Notes:}This table presents the coefficients reflecting the impact of agent type on the various AI based creativity criteria scores. ***, ** and * indicate significance at the 1\%, 5\% and 10\% level, respectively. Effects are estimated using an Ordered Polynomial Logit for Validity and OLS for other variables. \end{tablenotes}
 \end{threeparttable}
 }
\end{table} 
